Updated Standard for Secure Satellite Communications: Analysis of Satellites, Attack Vectors, Existing Standards, and Enterprise and Security Architectures

Satellites play a vital role in remote communication where traditional communication mediums struggle to provide benefits over associated costs and efficiency. In recent years, satellite communication has achieved utter interest in the industry due to the achievement of high data rates through the massive deployment of LEO satellites. Because of the complex diversity in types of satellites, communication methodologies, technological obstacles, environmental limitations, elements in the entire ecosystem, massive financial impact, geopolitical conflict and domination, easier access to satellite communications, and various other reasons, the threat vectors are rising in the threat landscape. To achieve resilience against those, only technological solutions are not enough. An effective approach will be through security standards. However, there is a considerable gap in the industry regarding a generic security standard framework for satellite communication and space data systems. A few countries and space agencies have their own standard framework and private policies. However, many of those are either private, serve the specific requirements of specific missions, or have not been updated for a long time. This project report will focus on identifying, categorizing, comparing, and assessing elements, threat landscape, enterprise security architectures, and available public standards of satellite communication and space data systems. After that, it will utilize the knowledge to propose an updated standard framework for secure satellite communications and space data systems.

==> Chapters/Formatting.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Background}
Satellites are a crucial element in remote wireless communication where it is difficult to reach through other traditional communication mediums like cable or fiber. From a commercial vessel floating in the middle of the ocean to personal internet connection, the demand for satellite communication is increasing day by day to gain better coverage and high-volume data transfer ability. 

Satellites can be used for various purposes. The most common usage is for television broadcasting where a large coverage is necessary. With satellites, television programs can be broadcasted over multiple countries and region at the same time. Telecommunication is another significant usage of satellites. It makes telecommunication possible after a natural disaster when other communication mediums face failure. It also enables communication to the areas which are extremely challenging to reach over conventional communication mediums like maritime ships or military vehicles in the middle of the ocean. If there is a clear path between the telecommunication user and the satellite (as the microwave energy travels in a straight line), a close connection can be established without requiring any repeaters to boost the signal in between. It removes the necessity of installing repeaters to maintain the line-of-sight for sending or receiving microwave signals to/from large distances.

Another popular use of satellites is for providing broadband internet connectivity. In long distance cable connection, specific repeaters have to be deployed to amply the signal due to the energy loss during signal transfer. This is financially not profitable while establishing a connection to remote locations. Besides communicating over satellites, maritime vessels also heavily use satellites for Global Positioning System (GPS) based navigation. Another significant usage of satellites is collecting weather information from the space. It enables monitoring weather conditions from a global perspective.

Satellites are also an important source of environmental information. Satellites orbiting the earth can continuously send environmental and climate information which can be stored and analyzed to predict climate changes in the future and identify pattern in climate change. Another significant arena of satellites is space research. Before launching satellites, all space observation was done from ground telescopes, radars, and other ground-based specialized hardware receivers. Up until today, more than 50 satellites have been launched to the space which were used for collecting information about the space. Two most significant satellite telescopes are the Hubble Space Telescope [4] and the James Webb Space Telescope [5] which have immense contribution to the space knowledge we have gathered up until now. Militaries of different countries also heavily use satellite-based communication for collecting real-time accurate intelligence from their field agents. They also use satellites for accurately guiding weapons and aircrafts from a long distance.

On top of everything, to utilize the advantages of satellites, organizations do not need to deploy their own satellite in the space by investing a significantly large amount of money. Rather, smaller organizations, even individuals, can rent the satellite capacity from other organizations who have deployed satellites up in the space. Ground stations or receivers can be deployed at multiple locations very quicky and cost-effectively to establish a connection to the satellites. The receivers today can be as small as a handheld device. A majority of the satellites in the space are basically a microwave signal repeater that relays the signal sent from the ground-based stations. However, observatory and other type of satellites generation information and then send them to the ground stations instead of relaying. Jeffrey Bardin [42] identified that the largest usage of satellites is by the business communication users. The other prominent users are the military and civil communication users. This is demonstrated in \ref{fig:share_of_usage_percentage}.

\begin{figure}[h!]
    \centering
        \includegraphics[scale=0.7]{Figures/share_of_usage_percentage.png}
        \caption{Share of satellite usage by various industries}
        \label{fig:share_of_usage_percentage}
\end{figure}

Each sector depending on Satellite communication has its own huge share in business. For example, the shipping industry alone is responsible for 90\% of the trades in the world [1] which heavily depends on Global Navigation Satellite Systems (GNSS) [2]. As per the GrandViewResearch report [6], the overall market size of Satellite Communication in 2022 is USD 77.10 Billion and consolidated revenue in Satellite Communication is expected to be USD 159.50 Billion. The compound annual growth rate (CAGR) is 9.5\% from the year 2022 to 2030 based on the historical data from the year 2017 to 2020. FortuneBusinessInsights also forecasted the same 9.54\% CAGR for the period of year 2022 to 2029 [7]. Besides government and military, telecommunication and broadcasting media sectors have been occupying a significant portion of the user base in satellite communication. To achieve global connectivity objectives, private business organizations are investing more into satellite communication sector. In the 1990s, narrow band Satellites were introduced and that initialized the commercialization and privatization of Satellite usage [11]. In today's world, satellite-based communication is considered to be a significant part of 5G advancement (B5G) and 6G communication standards [12].

Depending on the distance of the satellite from the earth ground level, some satellites can cover up to one third of the entire earth area at the same time. For an example, a Geostationary Satellite can have coverage over 40 degrees of latitude on earth [10]. Due this unchallenged advantage, researchers and domain experts have always been working hard to further develop this communication medium. Since the beginning of the journey, satellite technologies kept evolving to meet the demand in the industry. With recent development of technologies and advancement and with heavy investment from private business sectors, satellite communication now allows users to achieve gigabit speed in personal communication and transferring data through satellites without managing long cables and expensive infrastructure. The upcoming O3b mPOWER constellation will be able to provide up to multiple gigabytes per second towards a single user [14]. In summer 2021, NASA has showcased the dynamic power of laser-based communication for satellites which will be capable of transmitting more data than ever before [15].

As per the European Space Agency report released on 2022 [9], a record number of rockets flew to the space to put multiple satellites in the orbit. This is likely to be increased in the upcoming year taking the market size expansion in consideration based on the CAGR. Since the first trial of Satellite Communication at the Tokyo Olympics 1964 [11], the use of Satellites kept increasing. More and more countries are becoming interested in Satellites. \ref{fig:satellite_countries_1966} and \ref{fig:satellite_countries_2020} provides a clear representation of increased interest in satellites usage among state nations from the year 1966 to the year 2020.

\begin{figure}[ht]
    \centering
        \includegraphics[scale=1]{Figures/satellite_countries_1966.png}
        \caption{Countries involved with Satellites in year 1966}
        \label{fig:satellite_countries_1966}
\end{figure}

\begin{figure}[htbp]
    \centering
        \includegraphics[scale=1]{Figures/satellite_countries_2020.png}
        \caption{Countries involved with Satellites in year 2020}
        \label{fig:satellite_countries_2020}
\end{figure}

\begin{figure}[ht]
    \centering
        \includegraphics[scale=0.34]{Figures/satellited_launched_by_country.png}
        \caption{Satellites launched by countries until 2016}
        \label{fig:satellite_launch_countries}
\end{figure}

\begin{figure}[htbp]
    \centering
        \includegraphics[scale=0.365]{Figures/satellited_launched_by_type.png}
        \caption{Satellites launched by types until 2016}
        \label{fig:satellite_launch_type}
\end{figure}

%----------------------------------------------------------------------------------------

\section{Motivation}

Based on the dependence on satellite communication and significant financial impact, an attack on satellite communication can have catastrophic adverse effect ranging from financial damage to the loss of individual lives. Because of the possible wideness of impacts and weakness in legacy and costly infrastructure of satellite communications, adversaries are showing increased interest in attacking the satellite communications. All three core security services – Confidentiality, Integrity and Availability can be attacked in Satellite communications. If data is not encrypted with strong algorithm, confidentiality can be impacted. If appropriate cryptographic mechanism is not deployed, integrity can be affected. Recent research has proved that denial of service attack is possible, even on the latest technology implemented by the private commercial organization – SpaceX [13]. Satellite communication utilize the wireless communication link due to the architecture of this medium. Besides the common attacks on wireless networks, satellite communication is susceptible to spoofing, jamming signal-level attacks, data-level attacks [16], information-theoretic attacks, cryptographic attacks [3], physical layer attack, network layer attacks, denial of service attacks and many more. Several research over the past few decades have proposed different mitigation strategies for the aforementioned attacks.

However, there is a significant scope for risk management analysis and mitigation plan management towards the cyber security of Satellite Communication. This report will utilize the ISO/IEC 27001 and ISO/IEC 27005 standard frameworks to analyze the risks of the possible attacks and a pragmatic feasibility analysis of previously proposed mitigation strategies.

Moreover, the author was privileged to be one of the 18 people from the whole United Kingdom invited by the National Cyber Security Center (NCSC) UK for a workshop. The main focus of the workshop was on the security of satellite communications. This clearly resembles the interest of the government of the United Kingdom and the importance of securing satellite communications and portrays the impact of it in the upcoming decade.

\section{Objectives}
\begin{itemize}
  \item \textbf{Identification and Categorization of Satellites.} Identification and Categorization of Satellites.
  \item \textbf{Communication Development Timeline.} Timeline of Satellite Communication Development
  \item \textbf{Identification and Categorization of Threats.} Identification and Categorizations of Satellite Communication Threats
  \item \textbf{Mitigation Strategies.} Mitigation Strategies for the Satellite Communication Threats
  \item \textbf{Existing Standard Analysis.} Analyze Existing Standards for Satellite Communications and Space Data Systems
  \item \textbf{Propose Updated Standard.} Development of an Updated Satellite Communication Standard Framework
\end{itemize}

\section{Structure of the Project}
At first, this project focused on a literature review of previous research and publications to develop an overall understanding of the proposed security solutions for securing satellite communications. Upon review, it established the hypothesis that there is no single solution that can help in securing the diversified areas and requirements of satellite communications which is discussed in the literature review section of this report. The only pragmatic solution is developing a robust standard with a framework that can be applied by all the space organizations. Due to the rapid and ever-changing threat landscape, that standard has to be updated frequently to keep up with the security challenges in this domain.

Then to strengthen this hypothesis, this report conveyed an open survey to consider the opinions of the domain experts and associates in the cyber security field. The feedback of the survey is attached to this report. The findings from the survey strongly supports this hypothesis that a robust standard framework developed in collaboration with the militaries, governments and space agencies can help best in approaching security in satellite communication. Details of the survey is discussed in the following section.

For proposing an updated standard for secure satellite communication, this report needed a good understanding of the elements and segments in satellite communication. Through literature review, this report identified and categorized the core elements and segments of generic satellite communication. Then to further understanding the communication over the satellites, it required to identify and categorized the types of satellites which are already deployed in the space. This report researched and identified the types of satellites and their purposes. This enormously helped in understanding the elements involved in satellite communication and thus developing the proposed framework covering all the core elements of the framework. This is discussed in section 2.1 of this report.

To understand how the threats developed over the years since the beginning of satellite communication, this report researched on the evolution of satellites and satellite communications. It developed a timeline of satellite development since the beginning in the year 1945 until this year 2023. This is presented in section 2.2.

Another important area this report wanted to explore is the lifetime of satellites. This is significantly important while designing security around satellite communication for quite a few reasons. First of all, satellites with prolonged lifetime stays up in the space for even a decade. However, the threat landscape increases rapidly over the years. As a result, a mission with longer lifespan has to be robust enough to stay secure in the long run. Secondly, it's not cost effective and pragmatic to update major things on the satellite itself which is travelling thousands of kilometers per hour at an altitude of hundreds of miles above the ground. Because of these reasons, this report wanted to explore the lifetime of the significant satellites which are already deployed on the space. This particularly helps to understand for how long in average the communication has to stay resilient against the adversaries. This report doesn't suggest staying secure for a particular period. A system should be designed in such a way that it stays as much resilient as possible against the adversaries during the lifetime of the mission. However, while designing the mission security, a satellite having a few days of lifetime vs a satellite having a few decades of operation may require significantly different approach based on the requirements of the mission. A grant chart of satellite deployment and their lifetime is demonstrated in Section 2.3 of this report.

Once a good understanding of satellite elements, segments, evolution of satellites and lifetime is achieved, this report focused on understanding the attack vectors on satellites and satellite communications. This report not only researched on cyber-attacks but also researched on kinetic attacks. However, mitigation proposals for kinetic attacks are beyond the scope of this report. Attacks on satellite communications are described in Section 3.
As this report has developed the hypothesis at this point, the report proceeds in analyzing available standards for secure satellite communication. Surprisingly this report discovers that there is no updated available generic standard that specifically serves the interest of the United Kingdom and ally nation states.  Analysis of existing significant standards are described on Section 4.

Then on Section 5, this report proposes an updated standard for secure satellite communications and space data systems.

\section{Literature Review}
Satellite communication started way back in 1958 as part of a US Government project - SCORE (Signal Communication by Orbiting Relay Equipment) [4]. Since then, this communication medium has been used continuously through different other satellites and by satellite communication service providers including multiple governments and private organizations for satellite communication including maritime communication, global positioning, weather forecasting, military communication, etc. [5]). The available consumer mobile handsets are now capable of connecting through the 5G communication medium. The European Space Agency was considering the integration of satellite communication capabilities within the 5G spectrum [14]. Satellite communication will also play a vital role in the upcoming 6G communication (Saeed et al, 2021). 5465 artificial satellites are orbiting around the earth as of April 30, 2022 ( Number of Satellites in Space in 2022 , 2023). The European Space Agency categorized all these satellites into 6 major categories based on their orbits - GEO, LEO, MEO, SSO, GTO, and L-points [2]. The satellite communication market is expected to reach USD 41.86 Billion by 2025 [9]. Moreover, the value of the assets depending on GNSS (Global Navigation Satellite System) alone is around 800 Billion Euros as per the EC (European Commission) survey [13]. Because of the financial impact, this communication medium has acquired increased attention from attackers. According to James Turgal, the managing director of Cyber Risk Services at Deloitte, the human factor and the supply chain are the main areas of concern for cyber security around satellite communication [3]. That is why this report will analyze the possible and effective manners of securing satellite communication only from the ground station to the satellites but also will discuss the human factors revolving around the security in satellite communication. Different methods of cyber-attack are possible with the current satellite communication technology [10].

The current satellite communication has a wide variety of vulnerabilities including, but not limited to, backdoors, hardcoded credentials, insecure protocol, jamming, spoofing, and hijacking [11]. Among them, some attacks are intentional, but some are unintentional. For example, some amateur radio services, terrestrial video broadcasting signals (DVB-T), multicarrier modulated satellite communication systems, etc. can cause out-of-band interference unintentionally. However, previous research was on specific areas of the complex and large satellite communication systems instead of the security as a whole for the satellite communications and space data systems.

\section{Research Methodology}
This project follows the "Analytical" approach described in the MSc. Information Security Project Handbook 2022/2023 version 1.2 that was published in January 2023, Section 1.1. The project handbook mentions assessing standardization work under the "Analytical" paragraph in the aforementioned section. The end goal of this MSc. project is analyzing the current satellite communication security standard BS ISO 20214:2015 titled "Space data and information transfer systems — Security architecture for space data systems" and propose an updated standard for secure satellite communications and space data systems.

\section{Survey Data Analysis}
This project developed a set of questionnaires to collect generic opinion regarding satellite communication security. The questions and the answer choices were intentionally kept open to make it more inclusive. This provided the opportunity to acquire feedback from people from diversified demographic. The feedback was provided from people of:
\begin{itemize}
    \item Different age group
    \item Different educational qualifications
    \item Different organizations
    \item Different field of work domains
    \item Different countries
\end{itemize}

\begin{figure}
    \centering
      \begin{tikzpicture}
        \pie{19/45+ Years, 28/15 - 25 Years, 32/25 - 35 Years, 21/35 - 45 Years}
    \end{tikzpicture}  
    \caption{Survey Participants Age Groups}
    \label{fig:participants_age_group}
\end{figure}

Among the participants, 67\% had at least one postgraduate degree, 26\% had undergraduate degree and 7\% either had a PhD degree or a current PhD student.

Age Group Analysis is presented in \ref{fig:participants_age_group}

\begin{itemize}
    \item 28\% were between 15 - 25 years old
    \item 3\% were between 25 - 35 years old
    \item 21\% were between 35 - 45 years old
    \item 19\% were above 45 years old
\end{itemize}

The participants were from 29 different organization as specified in \ref{tab:participating_organizations}.

\begin{table}
\centering
\begin{tabular}{l l l}
\midrule
National Cyber Security Agency (NCSC), UK & Ministry of Defense (MoD), UK\\
GitHub (Microsoft) & KPMG\\
BP & Mission Aviation Fellowship (MAF), UK\\
BAE Systems & Liberty Global\\
Royal Holloway, University of London & Utrecht University\\
Northumbria University & University of Kent\\
University of Westminster & De Montfort University\\
Georgetown University & Coventry University\\
Undisclosed Security Consultancy Company & Bylor LTD\\
Alstom & Gemeente Alphen aan den Rijn\\
Tonnik Consulting & Thought Machine\\
STM & Sky\\
Babylon Health, UK & Mambu\\
CDW, UK\\
\bottomrule\\
\end{tabular}
\caption{Organizations of the participants in the survey}
\label{tab:participating_organizations}
\end{table}

Participants were from a diversified professional domain including – Cybersecurity, Information Security, Security and Compliance, Information Technology, Finance, University Lecturer, Mathematics, Business Information Systems, Business Management, Strategic Management, Engineering, Developer, Software Architect.
The survey acquired feedback from participants within geographically diversified areas. It recorded responses from countries including England, Qatar, Germany, Netherlands, Northern Ireland, Greece, USA, India, and UAE.

To understand the participants' perception regarding dependence on satellite communication, the survey asked if they have travelled by air in last 3 years. 86\% of the participants confirmed that they have did and 14\% did not. This will help in understanding the following area where the participants were asked if they think they will be impacted if a major attack happens on satellite communication.
For similar reason, participants were asked if they ordered any product which was shipped from abroad in last 3 years. 77\% participants confirmed that they did while 19\% didn't and 5\% cannot confirm.

These responses are significant because aviation and maritime industry heavily depends on satellite communications and any major attack on satellite communication can disrupt daily operation of these industries affecting millions of people including the participants of this survey.

Another very common usage of satellite is broadcasting television programs. According to the survey response, even today, 67\% of the participants or their neighbors have a satellite dish connected to their house for satellite TV. This resembles a big percentage of people still using satellite communications every day for entertainment and information purposes. Any adversarial impact (e.g., signal hijacking to spread propaganda which is described in detail later in this report) may include these audience and millions of others throughout the world.

Then the survey asked the participants how severely they think they will be impacted if a major attack happens on the mainstream satellite communication network. They were asked to rate it on a scale of 1 to 10 where 1 meaning not impacted at all and 10 meaning severely impacted. The average rating recorded is 6.91 as presented in \ref{fig:impact_score}. This indicates that the general public is aware that they will be considerably impacted if a major attack happens on the mainstream satellite communication network.

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis} [
        ybar,
        bar width=15pt,
        ylabel=Number of Participants,
        xlabel=Impact Score,
        ymax = 13
    ]
    \addplot[
        color=orange,
        fill=orange
    ] coordinates {
        (1,2) 
        (2,2) 
        (3,1) 
        (4,2)
        (5,5)
        (6,6)
        (7,2)
        (8,11)
        (9,3)
        (10,9)
    };
    \legend {Average 6.91};
    \end{axis}
    \end{tikzpicture}
    \caption{Impact of attacks on Satellite Communications}
    \label{fig:impact_score}
\end{figure}

The survey also asked them how dependent they are on satellite communications in their own understanding. In the similar way, they were asked to rate it on a scale of 1 to 10. 1 meaning not dependent at all and 10 meaning severely dependent. The average recorded rating is 7.02 which again indicates that they are aware of their dependence on satellite communication for their everyday activities as presented in \ref{fig:dependency_score}.

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis} [
        ybar,
        bar width=15pt,
        ylabel=Number of Participants,
        xlabel=Dependency Score,
        ymax = 11
    ]
    \addplot[
        color=cyan,
        fill=cyan
    ] coordinates {
        (1,1) 
        (2,0) 
        (3,3) 
        (4,3)
        (5,4)
        (6,7)
        (7,4)
        (8,8)
        (9,4)
        (10,9)
    };
    \legend {Average 7.02};
    \end{axis}
    \end{tikzpicture}
    \caption{Dependency on Satellite Communications}
    \label{fig:dependency_score}
\end{figure}

Now that it is clear that satellite communications have significant impacts on the life of people, the survey asked if they think "only" technological measures are enough to secure satellite communications. 16\% strongly disagree, 37\% disagree, 30\% were neutral and only 16\% agreed to this statement. This confirms that only technological controls are not enough to achieve resilience against the satellite communication threats.

In the next question, the survey asked the audience if they think governance and compliance are required to secure satellite communication. Not a single participant disagreed to this. 60\% agreed and 40\% strongly agreed to this.

The survey asked if militaries, governments, and space agencies of different countries should work together for developing standards in satellite communication. 51\% strongly agreed, 37\% agreed, 9\% were neutral and only 2\% disagreed with this. From the outcome, this report concludes that all the aforementioned concerns should work together to come up with a robust standard framework for securing satellite communications.

\section{Key Takeaways}
    \keyword{Considerable awareness} -- Majority of the audience understand that their everyday activities and business heavily depend on satellite communications.
    
    \keyword{Beyond technology} -- Only technological solutions are not enough to secure satellite communications.
    
    \keyword{Combined effort required} -- Governments, Militaries and Space Agencies should work together to develop standards for governing satellite communications to achieve resilience.

%----------------------------------------------------------------------------------------

\section{Getting Started with this Template}

If you are familiar with \LaTeX{}, then you should explore the directory structure of the template and then proceed to place your own information into the \emph{THESIS INFORMATION} block of the \file{main.tex} file. You can then modify the rest of this file to your unique specifications based on your degree/university. Section \ref{FillingFile} on page \pageref{FillingFile} will help you do this. Make sure you also read section \ref{ThesisConventions} about thesis conventions to get the most out of this template.

If you are new to \LaTeX{} it is recommended that you carry on reading through the rest of the information in this document.

Before you begin using this template you should ensure that its style complies with the thesis style guidelines imposed by your institution. In most cases this template style and layout will be suitable. If it is not, it may only require a small change to bring the template in line with your institution's recommendations. These modifications will need to be done on the \file{MastersDoctoralThesis.cls} file.

\subsection{About this Template}

This \LaTeX{} Thesis Template is originally based and created around a \LaTeX{} style file created by Steve R.\ Gunn from the University of Southampton (UK), department of Electronics and Computer Science. You can find his original thesis style file at his site, here:
\url{http://www.ecs.soton.ac.uk/~srg/softwaretools/document/templates/}

Steve's \file{ecsthesis.cls} was then taken by Sunil Patel who modified it by creating a skeleton framework and folder structure to place the thesis files in. The resulting template can be found on Sunil's site here:
\url{http://www.sunilpatel.co.uk/thesis-template}

Sunil's template was made available through \url{http://www.LaTeXTemplates.com} where it was modified many times based on user requests and questions. Version 2.0 and onwards of this template represents a major modification to Sunil's template and is, in fact, hardly recognisable. The work to make version 2.0 possible was carried out by \href{mailto:vel@latextemplates.com}{Vel} and Johannes Böttcher.

%----------------------------------------------------------------------------------------

\section{What this Template Includes}

\subsection{Folders}

This template comes as a single zip file that expands out to several files and folders. The folder names are mostly self-explanatory:

\keyword{Appendices} -- this is the folder where you put the appendices. Each appendix should go into its own separate \file{.tex} file. An example and template are included in the directory.

This chapter layout is specialised for the experimental sciences, your discipline may be different.

\keyword{Figures} -- this folder contains all figures for the thesis. These are the final images that will go into the thesis document.

\section{Filling in Your Information in the \file{main.tex} File}\label{FillingFile}

You will need to personalise the thesis template and make it your own by filling in your own information. This is done by editing the \file{main.tex} file in a text editor or your favourite LaTeX environment.

Open the file and scroll down to the third large block titled \emph{THESIS INFORMATION} where you can see the entries for \emph{University Name}, \emph{Department Name}, etc \ldots

Fill out the information about yourself, your group and institution. You can also insert web links, if you do, make sure you use the full URL, including the \code{http://} for this. If you don't want these to be linked, simply remove the \verb|\href{url}{name}| and only leave the name.

When you have done this, save the file and recompile \code{main.tex}. All the information you filled in should now be in the PDF, complete with web links. You can now begin your thesis proper!

%----------------------------------------------------------------------------------------

\section{The \code{main.tex} File Explained}

The \file{main.tex} file contains the structure of the thesis. There are plenty of written comments that explain what pages, sections and formatting the \LaTeX{} code is creating. Each major document element is divided into commented blocks with titles in all capitals to make it obvious what the following bit of code is doing. Initially there seems to be a lot of \LaTeX{} code, but this is all formatting, and it has all been taken care of so you don't have to do it.

Finally, there is the block where the chapters are included. Uncomment the lines (delete the \code{\%} character) as you write the chapters. Each chapter should be written in its own file and put into the \emph{Chapters} folder and named \file{Chapter1}, \file{Chapter2}, etc\ldots Similarly for the appendices, uncomment the lines as you need them. Each appendix should go into its own file and placed in the \emph{Appendices} folder.

After the preamble, chapters and appendices finally comes the bibliography. The bibliography style (called \option{authoryear}) is used for the bibliography and is a fully featured style that will even include links to where the referenced paper can be found online. Do not underestimate how grateful your reader will be to find that a reference to a paper is just a click away. Of course, this relies on you putting the URL information into the BibTeX file in the first place.

%----------------------------------------------------------------------------------------

\section{Thesis Features and Conventions}\label{ThesisConventions}

To get the best out of this template, there are a few conventions that you may want to follow.

One of the most important (and most difficult) things to keep track of in such a long document as a thesis is consistency. Using certain conventions and ways of doing things (such as using a Todo list) makes the job easier. Of course, all of these are optional and you can adopt your own method.

\subsection{Printing Format}

This thesis template is designed for double sided printing (i.e. content on the front and back of pages) as most theses are printed and bound this way. Switching to one sided printing is as simple as uncommenting the \option{oneside} option of the \code{documentclass} command at the top of the \file{main.tex} file. You may then wish to adjust the margins to suit specifications from your institution.

The headers for the pages contain the page number on the outer side (so it is easy to flick through to the page you want) and the chapter name on the inner side.

The text is set to 11 point by default with single line spacing, again, you can tune the text size and spacing should you want or need to using the options at the very start of \file{main.tex}. The spacing can be changed similarly by replacing the \option{singlespacing} with \option{onehalfspacing} or \option{doublespacing}.

\subsection{References}

The \code{biblatex} package is used to format the bibliography and inserts references such as this one \parencite{Reference1}. The options used in the \file{main.tex} file mean that the in-text citations of references are formatted with the author(s) listed with the date of the publication. Multiple references are separated by semicolons (e.g. \parencite{Reference2, Reference1}) and references with more than three authors only show the first author with \emph{et al.} indicating there are more authors (e.g. \parencite{Reference3}). This is done automatically for you. To see how you use references, have a look at the \file{Chapter1.tex} source file. Many reference managers allow you to simply drag the reference into the document as you type.

Scientific references should come \emph{before} the punctuation mark if there is one (such as a comma or period). The same goes for footnotes\footnote{Such as this footnote, here down at the bottom of the page.}. You can change this but the most important thing is to keep the convention consistent throughout the thesis. Footnotes themselves should be full, descriptive sentences (beginning with a capital letter and ending with a full stop). The APA6 states: \enquote{Footnote numbers should be superscripted, [...], following any punctuation mark except a dash.} The Chicago manual of style states: \enquote{A note number should be placed at the end of a sentence or clause. The number follows any punctuation mark except the dash, which it precedes. It follows a closing parenthesis.}

The bibliography is typeset with references listed in alphabetical order by the first author's last name. This is similar to the APA referencing style. To see how \LaTeX{} typesets the bibliography, have a look at the very end of this document (or just click on the reference number links in in-text citations).

\subsubsection{A Note on bibtex}

The bibtex backend used in the template by default does not correctly handle unicode character encoding (i.e. "international" characters). You may see a warning about this in the compilation log and, if your references contain unicode characters, they may not show up correctly or at all. The solution to this is to use the biber backend instead of the outdated bibtex backend. This is done by finding this in \file{main.tex}: \option{backend=bibtex} and changing it to \option{backend=biber}. You will then need to delete all auxiliary BibTeX files and navigate to the template directory in your terminal (command prompt). Once there, simply type \code{biber main} and biber will compile your bibliography. You can then compile \file{main.tex} as normal and your bibliography will be updated. An alternative is to set up your LaTeX editor to compile with biber instead of bibtex, see \href{http://tex.stackexchange.com/questions/154751/biblatex-with-biber-configuring-my-editor-to-avoid-undefined-citations/}{here} for how to do this for various editors.

\subsection{Tables}

Tables are an important way of displaying your results, below is an example table which was generated with this code:

{\small
\begin{verbatim}
\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}
\end{verbatim}
}

\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}

You can reference tables with \verb|\ref{<label>}| where the label is defined within the table environment. See \file{Chapter1.tex} for an example of the label and citation (e.g. Table~\ref{tab:treatments}).

\subsection{Figures}

There will hopefully be many figures in your thesis (that should be placed in the \emph{Figures} folder). The way to insert figures into your thesis is to use a code template like this:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}
\end{verbatim}
Also look in the source file. Putting this code into the source file produces the picture of the electron that you can see in the figure below.



Sometimes figures don't always appear where you write them in the source. The placement depends on how much space there is on the page for the figure. Sometimes there is not enough room to fit a figure directly where it should go (in relation to the text) and so \LaTeX{} puts it at the top of the next page. Positioning figures is the job of \LaTeX{} and so you should only worry about making them look good!

Figures usually should have captions just in case you need to refer to them (such as in Figure~). The \verb|\caption| command contains two parts, the first part, inside the square brackets is the title that will appear in the \emph{List of Figures}, and so should be short. The second part in the curly brackets should contain the longer and more descriptive caption text.

The \verb|\decoRule| command is optional and simply puts an aesthetic horizontal line below the image. If you do this for one image, do it for all of them.

\LaTeX{} is capable of using images in pdf, jpg and png format.

\subsection{Typesetting mathematics}

If your thesis is going to contain heavy mathematical content, be sure that \LaTeX{} will make it look beautiful, even though it won't be able to solve the equations for you.

The \enquote{Not So Short Introduction to \LaTeX} (available on \href{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}{CTAN}) should tell you everything you need to know for most cases of typesetting mathematics. If you need more information, a much more thorough mathematical guide is available from the AMS called, \enquote{A Short Math Guide to \LaTeX} and can be downloaded from:
\url{ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf}

There are many different \LaTeX{} symbols to remember, luckily you can find the most common symbols in \href{http://ctan.org/pkg/comprehensive}{The Comprehensive \LaTeX~Symbol List}.

You can write an equation, which is automatically given an equation number by \LaTeX{} like this:
\begin{verbatim}
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}
\end{verbatim}

This will produce Einstein's famous energy-matter equivalence equation:
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}

All equations you write (which are not in the middle of paragraph text) are automatically given equation numbers by \LaTeX{}. If you don't want a particular equation numbered, use the unnumbered form:
\begin{verbatim}
\[ a^{2}=4 \]
\end{verbatim}

%----------------------------------------------------------------------------------------

\section{Sectioning and Subsectioning}

You should break your thesis up into nice, bite-sized sections and subsections. \LaTeX{} automatically builds a table of Contents by looking at all the \verb|\chapter{}|, \verb|\section{}|  and \verb|\subsection{}| commands you write in the source.

The Table of Contents should only list the sections to three (3) levels. A \verb|chapter{}| is level zero (0). A \verb|\section{}| is level one (1) and so a \verb|\subsection{}| is level two (2). In your thesis it is likely that you will even use a \verb|subsubsection{}|, which is level three (3). The depth to which the Table of Contents is formatted is set within \file{MastersDoctoralThesis.cls}. If you need this changed, you can do it in \file{main.tex}.

%----------------------------------------------------------------------------------------

\section{In Closing}

You have reached the end of this mini-guide. You can now rename or overwrite this pdf file and begin writing your own \file{Chapter1.tex} and the rest of your thesis. The easy work of setting up the structure and framework has been taken care of for you. It's now your job to fill it out!

Good luck and have lots of fun!

\begin{flushright}
Guide written by ---\\
Sunil Patel: \href{http://www.sunilpatel.co.uk}{www.sunilpatel.co.uk}\\
Vel: \href{http://www.LaTeXTemplates.com}{LaTeXTemplates.com}
\end{flushright}

